CM-EVS: Sparse Panoramic RGB-D-Pose Data for Complete Scene Coverage

Modern 3D visual learning relies on observations sampled from metric 3D assets, yet existing scans, meshes, point clouds, simulations, and reconstructions do not directly provide a sparse, comparable, and geometry-consistent panoramic training interface. Dense trajectories duplicate nearby views, source-specific rendering policies yield heterogeneous annotations, and sparse heuristics may miss important regions or introduce depth-inconsistent observations. We study how to convert 3D assets into sparse panoramic RGB-D-pose data that preserves complete scene coverage with low redundancy and auditable provenance. We propose COVER (Coverage-Oriented Viewpoint curation with ERP Range-depth warping), a training-free ERP viewpoint curator that projects geometry observed from selected views into candidate ERP probes, scores incremental coverage, and penalizes depth conflicts. Under bounded proxy error, its greedy coverage proxy preserves the standard coverage-style approximation behavior up to an additive error term. Using COVER, we build CM-EVS (Coverage-curated Metric ERP View Set), a panoramic RGB-D-pose dataset with 36,373 curated ERP frames from 1,275 indoor scenes across Blender indoor, HM3D, and ScanNet++, complemented by outdoor panoramas from TartanGround and OB3D re-encoded into the same schema. Each frame provides full-sphere RGB, metric range depth, calibrated pose; COVER-produced indoor frames include per-step provenance logs. With a median of only 25 frames per indoor scene, CM-EVS covers all 13 unified room types while maintaining compact scene-level coverage. Experiments show that COVER improves the coverage-conflict trade-off, making CM-EVS a sparse, compact, and auditable RGB-D-pose resource for geometry-consistent panoramic 3D learning.

==> figures/1_CM_EVS_overview.tex <==

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/assets/F1_overview_of_CM-EVS.pdf}
\caption{\textbf{Overview of CM-EVS.} The release packages four complementary artifacts produced
under one principle --- \emph{maximize geometric coverage with the fewest ERP frames possible}:
(a)~a curated dataset of 11{,}583 ERP RGB--depth--pose frames across 326 Blender indoor scenes
(CC-BY 4.0) plus re-encoded TartanGround / OB3D outdoor frames, all under a single ERP +
world-to-camera pose schema; (b)~per-frame provenance metadata --- candidate set, coverage gain
$G_t$, depth-conflict ratio $L_t$, score $s_t$ --- shipped alongside every curator-produced
frame; (c)~license-aware adapter packages that regenerate matched HM3D / ScanNet++ frames
locally without redistributing gated assets; (d)~a training-free, depth-conflict-aware curator
with a $(1-1/e)$-style noisy-oracle approximation guarantee (Lemma~\ref{lem:noisy}). This
figure summarizes \emph{what is in the release}; the per-scene execution flow that produces a
single curated frame is depicted separately in Fig.~\ref{fig:pipeline}.}
\label{fig:1_CM_EVS_overview}
\end{figure}

==> sections/2_related_work.tex <==
\section{Related Work}
\label{sec:rw}

\paragraph{3D scene resources.}
Matterport3D \citep{chang2017matterport3d}, ScanNet \citep{dai2017scannet}, ScanNet++
\citep{yeshwanth2023scannetpp}, ARKitScenes \citep{dehghan2021arkitscenes}, HM3D
\citep{ramakrishnan2021hm3d}, and Replica \citep{straub2019replica} are the main 3D scene
resources we build on. Their camera trajectories are inherited from human operators or
delegated to downstream simulators. We treat them as \textbf{inputs} to CM-EVS rather than
competitors: HM3D and ScanNet++ are exposed through adapters, and we do not claim a new 3D
scene collection. Hypersim \citep{roberts2021hypersim}, Kubric \citep{greff2022kubric},
Infinigen \citep{raistrick2023infinigen}, 3D-FRONT \citep{fu20213dfront}, and
Structured3D \citep{zheng2020structured3d} couple their viewpoint policies to the rendering
backend; CM-EVS instead exposes the policy as a controlled, fixed-budget curator that runs
through \texttt{.blend}, \texttt{.glb}, and \texttt{.ply} adapters. Embodied-AI scene
platforms such as Gibson \citep{xia2018gibson} and iGibson \citep{shen2021igibson} similarly
treat camera trajectories as a downstream simulator concern rather than an auditable
release-time artifact.

\paragraph{Panoramic NeRF, Gaussian splatting, and NVS.}
Recent panoramic NeRF \citep{mildenhall2020nerf} and Gaussian-splatting
\citep{kerbl20233dgs} works --- including 360-GS
\citep{bai2024360gs}, EgoNeRF \citep{choi2023egonerf}, Omni-NeRF \citep{gu2022omninerf},
panoramic radiance fields (PERF \citep{wang2024perf}, PanoGRF \citep{chen2023panogrf},
360Roam \citep{huang2022360roam}), and panoramic-GS reconstruction pipelines
(e.g., DreamScene360 \citep{zhou2024dreamscene360}) --- have shown that ERP input is a viable
substrate for panoramic novel-view synthesis, but each paper assembles its own training data:
hand-held panoramic captures (e.g., OmniPhotos \citep{bertel2020omniphotos}), per-paper
Blender renders, or repurposed indoor-scan panoramas. The supply side --- a public, license-clean ERP RGB-D-pose corpus with calibrated
poses, ground-truth depth, and a unified coordinate convention --- has lagged behind the
modeling side. CM-EVS contributes on the supply side; it does not propose a new NVS model.

\paragraph{Panoramic generation.}
Pano3D \citep{albanis2021pano3d}, 360DVD \citep{wang2024360dvd}, DiffPano
\citep{ye2024diffpano}, Matrix-3D \citep{zhang2025matrix3d}, MVDiffusion
\citep{tang2023mvdiffusion}, Text2Light \citep{chen2022text2light}, PanFusion
\citep{zhang2024panfusion}, PanoDiffusion \citep{wu2024panodiffusion}, and follow-up
panoramic-generation work synthesize ERP content from
text, noise, or scripted trajectories. They are complementary to CM-EVS: CM-EVS provides
geometrically consistent ERP RGB-D-pose supervision drawn from explicit 3D assets, which can
be used to evaluate or to pretrain panoramic-generation models.

\paragraph{View planning and next-best-view.}
Classical NBV literature
\citep{connolly1985nbv,massios1998nbv,vasquez2014volumetric}, set-cover view planning
(SCVP) \citep{pan2022scvp}, and recent active-NeRF / learned-NBV approaches
(e.g., GenNBV \citep{chen2024gennbv}, ActiveNeRF \citep{pan2022activenerf},
NeurAR \citep{ran2023neurar}) target online reconstruction, inspection, or robot
exploration. CM-EVS is in a different regime: offline, training-free, fixed-budget
input-view selection over many existing scenes, with the policy exposed as an auditable
artifact rather than embedded in an online robot loop.

\paragraph{Dataset documentation practice.}
Following Datasheets for Datasets \citep{gebru2021datasheets}, the dataset ships with a complete
Datasheet (Appendix~\ref{app:datasheet}), Croissant metadata \citep{mlcommons2024croissant}
(Appendix~\ref{app:croissant}), license table (Appendix~\ref{app:license}), and a 50-frame audit
(Appendix~\ref{app:audit}). Where prior panoramic resources treat the camera-policy variable as
implicit, we make it the headline auditable field.

\paragraph{Position relative to existing resources.}
Table~\ref{tab:position} summarizes how CM-EVS differs from prior panoramic and 3D-scene resources
along the dimensions that matter for fixed-budget viewpoint comparison.

\begin{table}[h]
\caption{Position of CM-EVS relative to existing resources. \textbf{Frames/scene}
captures how aggressively a corpus emits viewpoints per scene unit; lower numbers, when
matched against scene-type coverage and modality completeness, indicate redundancy
control rather than data scarcity. CM-EVS sits one-to-two orders of magnitude below
ERP corpora that emit a fixed-per-scene budget. ``Audit. policy'' marks whether the
viewpoint selection policy is exposed as an auditable, citable artifact (per-step
logs of $G_t$, $L_t$, $s_t$ and the candidate set), rather than embedded in a
per-paper subsampling script.}
\label{tab:position}
\centering
\small
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llccccl}
\toprule
Resource & 3D source & ERP RGB-D-pose? & Frames / scene & Audit. policy & Fixed-$K$ bench. & Direct release \\
\midrule
Matterport3D            & real-scan mesh           & partial             & $\sim$120 & no  & no  & gated \\
ScanNet++               & real-scan mesh/cloud     & perspective         & $\sim$3{,}960 & no  & no  & gated \\
HM3D                    & real-scan mesh           & user-rendered       & user-set & no  & no  & gated \\
Hypersim                & synthetic                & perspective         & 168 & no  & no  & public \\
Kubric / Infinigen      & synthetic / procedural   & user-rendered       & user-set & part. & no & public gen. \\
360DVD                  & scripted video           & ERP RGB only        & 100 & no  & no  & mixed \\
Matrix-3D / Matrix-Pano & generative / scripted    & ERP RGB(-D)         & $\sim$138 & no  & no  & mixed \\
\textbf{CM-EVS (ours)}  & \texttt{.blend/.glb/.ply} & \textbf{ERP RGB-D-pose} & \textbf{$\sim$25 (median)} & \textbf{yes} & \textbf{yes} & CC-BY 4.0 + regen. \\
\bottomrule
\end{tabular}}
\end{table}



==> sections/2_related_work_2.tex <==
\section{Related Work}
\label{sec:rw}

\subsection{Panoramic Data for 3D Learning}

Panoramic RGB-D-pose observations provide a compact interface for 3D perception, reconstruction, and generation, since a single ERP frame captures a full $4\pi$ field of view under a unified spherical parameterization. Existing 3D scene resources, including Matterport3D~\citep{chang2017matterport3d}, ScanNet++~\citep{yeshwanth2023scannetpp}, HM3D~\citep{ramakrishnan2021hm3d}, Hypersim~\citep{roberts2021hypersim}, Structured3D~\citep{zheng2020structured3d}, TartanGround \citep{patel2025tartanground}, and OB3D \citep{ito2025ob3d}, provide rich geometry, annotations, or simulation environments. Panoramic datasets and benchmarks such as Pano3D~\citep{albanis2021pano3d}, 360DVD~\citep{wang2024360dvd}, Matrix-3D~\citep{zhang2025matrix3d}, and Holo360D~\citep{ou2026holo360d} further highlight the value of full-sphere observations for depth estimation, generation, and reconstruction.
However, these resources often inherit source-specific capture protocols, dense trajectories, or downstream rendering choices. As a result, equal frame counts may correspond to substantially different geometric evidence, and the camera policy behind a dataset is rarely exposed as a reproducible artifact. Panoramic reconstruction and generation methods, including PERF~\citep{wang2024perf}, PanoGRF~\citep{chen2023panogrf}, 360-GS~\citep{bai2024360gs}, DreamScene360~\citep{zhou2024dreamscene360}, Text2Light~\citep{chen2022text2light}, MVDiffusion~\citep{tang2023mvdiffusion}, DiffPano~\citep{ye2024diffpano}, and PanoDiffusion~\citep{wu2024panodiffusion}, advance model design, but typically rely on per-paper view construction pipelines. \emph{CM-EVS instead targets the data-supply layer: converting heterogeneous 3D assets into sparse, calibrated, and comparable panoramic RGB-D-pose observations.} \emph{Its goal is not to introduce another modeling benchmark alone, but to make the observation policy behind panoramic 3D learning explicit and auditable.}

\subsection{View Selection for Data Curation}

View planning and next-best-view methods study how to select camera poses that reveal new geometry or reduce reconstruction uncertainty~\citep{vasquez2014volumetric}. Recent learning-based approaches, such as SCVP~\citep{pan2022scvp}, ActiveNeRF~\citep{pan2022activenerf}, NeurAR~\citep{ran2023neurar}, and GenNBV~\citep{chen2024gennbv}, formulate view selection as an online policy for active reconstruction, exploration, or neural scene modeling. These methods are typically designed for agents interacting with unknown scenes, where the camera policy is part of the reconstruction process itself.
Our setting is complementary. \textsc{COVER} is an offline, training-free, fixed-budget curator for building panoramic training data from existing 3D assets. Rather than optimizing online exploration, it selects ERP viewpoints by balancing incremental scene coverage with depth-conflict penalties, exposing non-redundant geometry while avoiding inconsistent observations. CM-EVS further makes this policy auditable by releasing candidate pools, coverage gains, conflict ratios, selection scores, and provenance logs. \emph{This allows users to reproduce the released view policy, diagnose failure cases, or replace \textsc{COVER} with alternative strategies under the same candidate space.} \emph{The release follows \emph{Datasheets for Datasets}~\citep{gebru2021datasheets} and Croissant~\citep{mlcommons2024croissant}, positioning CM-EVS as a reproducible observation layer rather than a source-specific rendering recipe.}

==> sections/5_case_study.tex <==
\section{Case studies: what the curated frames look like}
\label{sec:case_study}

This section is an entirely qualitative show-and-tell. Each case visualises one of the
four properties of \S\ref{sec:datasetanalysis} on a real release scene without invoking a
single downstream metric. All figures and statistics are recoverable from
\texttt{metadata/per\_step\_log.jsonl} and the released frames; no model is trained, no
held-out subset is created, and no external benchmark is consulted.

\subsection{Multi-view consistency on a single Blender residential room}
\label{sec:case_multiview}

Figure~\ref{fig:case_multiview} fixes a Blender indoor residential scene and shows the
$K\!=\!6$ first selected viewpoints. For each viewpoint we display the ERP RGB, the range
depth, and a glyph indicating the world-to-camera pose (orientation arrow + position
relative to the AABB centre). The selected centres are spread across the scene's three
functional zones (entryway, living area, bedroom alcove); together they form a
multi-view scene observation in which every selected frame is itself a full $4\pi$ sample
rather than a slice of one. The accompanying footprint plot overlays the six camera
positions on the scene's accumulated point cloud, making the geometric coverage of the
selection set visible at a glance --- the same coverage that the curator's $G_t$ score
optimises step by step.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/assets/case_multiview.png}
\caption{Multi-view consistency on a Blender indoor residential scene. Six selected
viewpoints, each rendered as a full $4\pi$ ERP RGB + range-depth + pose glyph, with their
positions overlaid on the scene's accumulated point cloud (right). Together the six
viewpoints span three functional zones; each viewpoint individually contributes a complete
sphere of multi-view content rather than a perspective slice.}
\label{fig:case_multiview}
\end{figure}

\subsection{Cross-source diversity: same recipe, three rooms, three room-type buckets}
\label{sec:case_cross}

Figure~\ref{fig:case_cross_source} runs the same curator recipe ($\lambda\!=\!0.35$,
gain-gradient early stop, all defaults) on three scenes drawn from three sources and three
buckets of the unified room-type taxonomy: a Blender indoor commercial space (an
underrepresented category in real-scan campaigns), an HM3D residential bedroom, and a
ScanNet++ kitchen. For each scene we show two selected ERP RGB frames and the per-step
coverage-gain curve recovered from \texttt{metadata/per\_step\_log.jsonl}. The three
curves saturate at visibly different rates --- the commercial space takes longer to
plateau (more functional zones), the bedroom and kitchen plateau faster (single-purpose
layouts) --- which is exactly the scene-adaptive behaviour the gain-gradient early stop is
designed to expose. The visual contrast across rooms makes concrete the diversity claim
made by Figure~\ref{fig:xdataset_roomtype}: a single curator recipe routinely produces
Blender indoor commercial frames \emph{and} HM3D residential frames \emph{and} ScanNet++
kitchen frames, all under the same schema.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/assets/case_cross_source.png}
\caption{Cross-source diversity. Same curator recipe applied to a Blender indoor
commercial space, an HM3D residential bedroom, and a ScanNet++ kitchen. Two selected
ERP RGB frames per scene; per-step gain curves on the right. Saturation rates differ by
scene complexity, illustrating the gain-gradient early stop in action.}
\label{fig:case_cross_source}
\end{figure}

\subsection{Low redundancy in action: an open-plan office at $K\!=\!8$ vs.\ $K\!=\!30$}
\label{sec:case_low_redundancy}

Figure~\ref{fig:case_lowred} runs the curator on a large open-plan office scene under two
budgets: a budget-tight $K\!=\!8$ and a budget-loose $K\!=\!30$. We render the
$K\!=\!8$ frames as ERP thumbnails plus their footprint, and the $K\!=\!30$ frames as
their footprint over the same point cloud. Two observations stand out qualitatively.
First, the $K\!=\!8$ selection already covers all four functional zones of the open-plan
office (reception, meeting, workstation cluster, kitchenette); zoning coverage is
established by step $\approx\!6$ and the remaining two frames refine within zones.
Second, the $K\!=\!30$ selection at the same $\lambda$ continues to add frames inside
zones already covered by $K\!=\!8$, with marginal gain dropping below $\tau\!=\!1\%$
around $t\!\approx\!22$ --- the natural moment for the gain-gradient early stop to fire
in production. Both regimes are recoverable from the same release: the per-step log
records every candidate, score, and accumulated coverage so a downstream user can ask
``what would I have selected at $K\!=\!12$?'' without rerunning the curator.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/assets/case3-k=8vsk=30.png}
\caption{Low redundancy in action on an open-plan office scene.
\textbf{Top:} $K\!=\!8$ selection --- eight ERP thumbnails plus their footprint over the
scene's accumulated point cloud; zoning coverage is essentially complete by
$t\!\approx\!6$. \textbf{Bottom:} $K\!=\!30$ footprint over the same scene; the gain
gradient drops below the production threshold $\tau\!=\!1\%$ around $t\!\approx\!22$,
which is the natural early-stop point. Both regimes are recoverable from a single
\texttt{metadata/per\_step\_log.jsonl}.}
\label{fig:case_lowred}
\end{figure}

